UniPELT: A Unified Framework for Parameter-Efficient Language Model Tuning

Recent parameter-efficient language model tuning (PELT) methods manage to match the performance of fine-tuning with much fewer trainable parameters and perform especially well when training data is limited. However, different PELT methods may perform rather differently on the same task, making it nontrivial to select the most appropriate method for a specific task, especially considering the fast-growing number of new PELT methods and tasks. In light of model diversity and the difficulty of model selection, we propose a unified framework, UniPELT, which incorporates different PELT methods as submodules and learns to activate the ones that best suit the current data or task setup via gating mechanism. On the GLUE benchmark, UniPELT consistently achieves 1~4% gains compared to the best individual PELT method that it incorporates and even outperforms fine-tuning under different setups. Moreover, UniPELT generally surpasses the upper bound that takes the best performance of all its submodules used individually on each task, indicating that a mixture of multiple PELT methods may be inherently more effective than single methods.

==> space.tex <==




\subsection{Floats (tables and figures)}
\begin{itemize}
    \item floatsep (\the\floatsep): space left between floats.

    \item textfloatsep (\the\textfloatsep): space between last top float or first bottom float and the text.

    \item intextsep (\the\intextsep) : space left on top and bottom of an in-text [h] float.

    \item dbltextfloatsep (\the\dbltextfloatsep) is textfloatsep for 2 column output.

    \item dblfloatsep (\the\dblfloatsep) is floatsep for 2 column output.

    \item abovecaptionskip (\the\abovecaptionskip): space above caption

    \item belowcaptionskip (\the\belowcaptionskip): space below caption
\end{itemize}

\subsection{Maths}
\begin{itemize}
\item abovedisplayskip (\the\abovedisplayskip): space before maths
\item belowdisplayskip (\the\belowdisplayskip): space after maths
\item abovedisplayshortskip (\the\abovedisplayshortskip): If the equation is preceded by a “sufficiently short” line
\item belowdisplayshortskip (\the\belowdisplayshortskip): If the equation is preceded by a “sufficiently short” line
\item arraycolsep (\the\arraycolsep): gap between columns of an array

\end{itemize}

==> table_glue_prefix_len.tex <==

\begin{table}[t]
\centering
\resizebox{.99\columnwidth}{!}{
\begin{tabular}{l cccc}
\toprule


\textbf{Method} & \textbf{SST-2}  & \textbf{CoLA} &  \textbf{STS-B}  & \textbf{QQP}\\

\midrule

Prefix ($L=10$) & 60.87$_{12.47}$		 & 0.00$_{0.00}$		 & 57.69$_{0.02}$	 & 15.68$_{0.12}$	\\
Prefix ($L=50$) & {79.52}$_{1.21}$		 & 5.19$_{8.62}$		 & 7.15$_{10.37}$	 & 58.02$_{2.91}$	\\
Adapter & \textbf{80.48}$_{2.94}$	 & 2.02$_{4.04}$	 & {77.32}$_{1.54}$	 & {60.88}$_{4.00}$		\\
\ours & 77.22$_{3.75}$	 & \textbf{14.42}$_{10.24}$			 & \textbf{79.14}$_{1.97}$	 & \textbf{63.41}$_{1.44}$		\\

\bottomrule
\end{tabular}}
\upv
\caption{Performance changes when increasing prefix length $L$ to match the trainable parameters of adapter.} 
\label{table_glue_prefix_len}
\downv
\end{table}
